Efficient-Adam: Communication-Efficient Distributed Adam

Distributed adaptive stochastic gradient methods have been widely used for large-scale nonconvex optimization, such as training deep learning models. However, their communication complexity on finding $\varepsilon$-stationary points has rarely been analyzed in the nonconvex setting. In this work, we present a novel communication-efficient distributed Adam in the parameter-server model for stochastic nonconvex optimization, dubbed {\em Efficient-Adam}. Specifically, we incorporate a two-way quantization scheme into Efficient-Adam to reduce the communication cost between the workers and server. Simultaneously, we adopt a two-way error feedback strategy to reduce the biases caused by the two-way quantization on both the server and workers, respectively. In addition, we establish the iteration complexity for the proposed Efficient-Adam with a class of quantization operators, and further characterize its communication complexity between the server and workers when an $\varepsilon$-stationary point is achieved. Finally, we apply Efficient-Adam to solve a toy stochastic convex optimization problem and train deep learning models on real-world vision and language tasks. Extensive experiments together with a theoretical guarantee justify the merits of Efficient Adam.

==> texfiles/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ccl.jpg}}]{Congliang Chen} received the B.S degree in computer science and technology from Peking University, China in 2018. He is working towards a Ph.D. degree of the Computer Information and Engineering at the School of Science and Engineering in the Chinese University of Hong Kong (Shenzhen). His research interest includes distributed optimization, federated learning and machine learning algorithms.
\end{IEEEbiography}

 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{shenli.png}}]{Li Shen} received his Ph.D. in school of mathematics, South China University of Technology in 2017. He is currently a research scientist at JD Explore Academy, China. Previously, he was a research scientist at Tencent AI Lab, China. His research interests include theory and algorithms for large scale convex/nonconvex/minimax optimization problems, and their applications in statistical machine learning, deep learning, reinforcement learning, and game theory.
\end{IEEEbiography}
 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{liuwei.png}}]{Wei Liu } (M'14-SM'19-F'23) received the Ph.D. degree from Columbia University in 2012 in Electrical Engineering and Computer Science. He is currently a Distinguished Scientist of Tencent and the Director of Ads Multimedia AI at Tencent Data Platform. Prior to that, he has been a research staff member of IBM T. J. Watson Research Center, USA from 2012 to 2015. Dr. Liu has long been devoted to fundamental research and technological development in core fields of AI, including deep learning, machine learning, reinforcement learning, computer vision, information retrieval, big data, etc. To date, he has published extensively in these fields with more than 280 peer-reviewed technical papers, and also issued over 30 US patents. He currently serves on the editorial boards of internationally leading AI journals like IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI), IEEE Transactions on Neural Networks and Learning Systems (TNNLS),  and IEEE Intelligent Systems. He is an Area Chair of top-tier computer science and AI conferences, e.g., NeurIPS, ICML, IEEE CVPR, IEEE ICCV, IJCAI, and AAAI. Dr. Liu is a Fellow of the IEEE, IAPR, and IMA, and an Elected Member of the ISI.   
\end{IEEEbiography}

 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{tom luo.jpg}}]{Zhi-Quan Luo} received the B.S. degree in applied mathematics from Peking University, China, and the Ph.D. degree in operations research from MIT in 1989. From 1989 to 2003, he held a faculty position with the ECE Department of McMaster University, Canada. He held a tier-1 Canada Research Chair in information processing from 2001 to 2003. After that, he has been a full professor at the ECE Department, University of Minnesota and held an endowed ADC Chair in digital technology. Currently, he is the Vice President (Academic) of the Chinese University of Hong Kong (Shenzhen) and the director of Shenzhen Research Institute of Big Data (SRIBD). Prof. Luo is a Fellow of IEEE and SIAM. He was elected to Fellow of Royal Society of Canada in 2014 and a Foreign Member of the Chinese Academy of Engineering (CAE) in 2021. He received four best paper awards from the IEEE Signal Processing Society, one best paper award from EUSIPCO, the Farkas Prize from INFORMS and the prize of Paul Y. Tseng Memorial Lectureship in Continuous Optimization as well as some best paper awards from international conferences. In 2021, he was awarded 2020 ICCM Best Paper Award by International Consortium of Chinese Mathematicians. He has published over 350 refereed papers, books and special issues. Prof. Luo has served as an Associate Editor for many internationally recognized journals and the Editor in Chief for IEEE Transactions on Signal Processing. His research mainly addresses mathematical issues in information sciences, with particular focus on the design, analysis and applications of large-scale optimization algorithms. (Email: luozq@cuhk.edu.cn)
\end{IEEEbiography}


==> texfiles/efficient_Adam_proof.tex <==
\section{Efficient Adam}\label{efficient-adam-sec}

In this section, we describe the proposed Efficient-Adam, whose workflow has already been displayed in Figure \ref{parameter-server}. To make the presentation clear, we split Efficient-Adam into two parts: parameter server part (Algorithm \ref{alg1}) and $N$-workers part (Algorithm \ref{alg2}). To reduce the communication overhead among the server and workers, we introduce a two-way quantization mapping. We denote the quantization function in the parameter server as $\mathcal{Q}_s(\cdot)$ and the quantization function in the  workers as $\mathcal{Q}_w(\cdot)$, respectively. The detailed iterations of Efficient-Adam are presented in the following. 

\begin{wrapfigure}{r}{0.50\textwidth}
\begin{minipage}{0.50\textwidth}
\vspace{-0.4cm}
\begin{algorithm}[H]
\caption{\ Efficient-Adam: server}
\label{alg1}
{\bf Parameters:} Choose quantization mapping $\mathcal{Q}_s(\cdot)$ 
via Definition \ref{quantization-mapping-def}. {Initialize $x_1 \in \mathbb{X}$ and error term $e_1=0$}.
\begin{algorithmic}[1]
\STATE Broadcasting $x_1$ to all workers;
\FOR{$t =1,2,\cdots,T$}
\STATE Gathering and averaging all updates from workers $\hat{\delta}_t = \frac{1}{N}\sum_{i = 1}^N \delta_t^{(i)}$;
\STATE Broadcasting $\tilde{\delta}_t = \mathcal{Q}_s(\hat{\delta}_t + e_t)$;
\STATE $e_{t+1} = \hat{\delta}_t + e_t - \tilde{\delta}_t$;
\STATE $x_{t+1} = x_{t}-\tilde{\delta}_t$;
\ENDFOR
\end{algorithmic}
{\bf Output:} $x_{T+1}$.
\end{algorithm}
\end{minipage}
\end{wrapfigure}
In the parameter server (see Algorithm \ref{alg1}), the initial value of $x$ will be broadcast to each worker at the initialization phase. Then in each iteration, the server gathers the update from each worker, calculates the average of these updates, and then broadcasts this average after a quantization function.

In each worker (see Algorithm \ref{alg2}), at the initial phase, the initial value of $x$ will be received. In each update iteration, a worker will sample a stochastic gradient $g_t$ and calculate the update vector $\delta_t$. Then it will send the update vector to the server with a quantization mapping and receive the average update vector from the server. Finally, the worker will update its local parameters. 
\hfill
\begin{wrapfigure}{r}{0.53\textwidth}
\begin{minipage}{0.53\textwidth}
\vspace{-0.85cm}
\begin{algorithm}[H]
\caption{\ Efficient-Adam: $i$-th worker}
\label{alg2}
{\bf Parameters:} Choose hyperparameters $\{\alpha_t\},\beta,\{\theta_t\}$, and quantization mapping $\mathcal{Q}_w(\cdot)$ satisfying Definition \ref{quantization-mapping-def}. Set initial values $m^{(i)}_0 = 0$ , $v^{(i)}_0 = \epsilon$, and error term $e^{(i)}_1 = 0$.
\begin{algorithmic}[1]
\STATE Receiving $x_1$ from the server;
\FOR{$t =1,2,\cdots,T$}
\STATE Sample a stochastic gradient of $f(x_t)$ as $g^{(i)}_t$;
\STATE $v^{(i)}_t = \theta_t v^{(i)}_{t-1} + (1-\theta_t) \big[g^{(i)}_t\big]^2$;
\STATE $m^{(i)}_t = \beta m^{(i)}_{t-1} + (1-\beta)g^{(i)}_t$;
\STATE Sending $\delta_t^{(i)} = \mathcal{Q}_w\left(\alpha_t{m^{(i)}_t}/{\sqrt{v^{(i)}_t}}+e^{(i)}_t\right)$;
\STATE $e^{(i)}_{t+1} = \alpha_t{m^{(i)}_t}/{\sqrt{v^{(i)}_t}}+e^{(i)}_t- \delta^{(i)}_t$;
\STATE Receiving $\tilde{\delta}_t$ from the server;
\STATE $x_{t+1} = x_t - \tilde{\delta}_t$;
\ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-0.8cm}
\end{wrapfigure}

\subsection{Complexity Analysis}

 In this subsection we give iteration complexity analysis and bit communication complexity analysis in order to obtain an $\varepsilon$-stationary solution of problem \eqref{problem} in Definition \ref{stationary-point-def}, i.e., $\mathbb{E}\|\nabla F(x)\|^2 \leq \varepsilon$. We denote $\delta_s$ and $\delta_s'$ as the constants defined in Definition \ref{quantization-mapping1} for $\mathcal{Q}_s()$, and $\delta_w$, $\delta_w'$ for $\mathcal{Q}_w()$. In addition, we further make another assumption on hyperparameters $\theta_t$ and $\alpha_t$.
 \begin{assumption}\label{hyper-parameters}
 For a given maximum number of iterations $T$, we define the exponential moving average parameter $\theta_t = 1-\frac{\theta}{T}$, and base learning rate $\alpha_t = \frac{\alpha}{\sqrt{T}}$. Besides, we define $\gamma = \beta/(1-\frac{\theta}{T})$. 
 \end{assumption} 

Below, we characterize the iteration complexity of Efficient-Adam to achieve an $\varepsilon$-stationary solution of problem \eqref{problem}. In the corollary, we characterize the overall bit communication complexity of Efficient-Adam with the quantization mapping defined in Example \ref{quantization-mapping3}. 

\begin{theorem}\label{complexity-quantization}
Let $\{x_t\}$ be the point generated by Algorithm \ref{alg1} and Algorithm \ref{alg2}. In addition, assume that all workers work identically and independently. Let $x_\tau^T$ be the random variable $x_\tau$ with $\tau$ taking from $\{1,2,\cdots, T\}$ with the same probability. For given $\varepsilon$, when $T\geq \frac{4(G^2+\epsilon d)}{(1-\beta)^2\alpha^2 \varepsilon^2}\left(F(x_1)-F^* + C_{2} \right)^2$, it always holds that
 \[
 \mathbb{E}[\|\nabla F(x_\tau^T)\|^2] \leq \varepsilon +  \left(\frac{\delta_s'}{\delta_s} +\frac{\delta_w'}{\delta_s\delta_w}\right)\frac{2L\sqrt{G^2+\epsilon d}C_3}{(1-\beta)},
 \] 
 where
$C_1 = \left(\frac{\beta/(1-\beta)}{\sqrt{(1-\gamma)\theta_1}}+1\right)^2$, $
C_{2} = \frac{d}{1-\sqrt{\gamma}}\left(\frac{\alpha^2L}{\theta(1-\sqrt{\gamma})^2\delta_w\delta_s} + \frac{2C_1G\alpha}{\sqrt{\theta}} \right) \left[\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{\theta}{1-\theta}\right]$, and $C_3 =\sqrt{\frac{d}{\theta(1-\sqrt{\gamma})^4}\left[\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{\theta}{1-\theta}\right]}.$
 \end{theorem}
 \begin{corollary}\label{bit-complexity-quantization}
 With the quantization function in Example \ref{quantization-mapping3}, when we want to get an $\varepsilon$-stationary solution we need at most $C_5$ bits per iteration on the workers and the server. Besides, to achieve an $\varepsilon$-stationary point, we need $\frac{16(G^2+\epsilon d)}{(1-\beta)^2\alpha^2 \varepsilon^2}\left(F(x_1)-F^* + C_{4} \right)^2$ iterations, where
$C_{4} = \frac{d}{1-\sqrt{\gamma}}\left(\frac{4\alpha^2L}{\theta(1-\sqrt{\gamma})^2} + \frac{2C_1G\alpha}{\sqrt{\theta}} \right) \left[\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{\theta}{1-\theta}\right]$, $C_5 = d\left(1+\log\left(\log(G)+\log\left(\frac{32Ld^2\sqrt{G^2\!+\!\epsilon d}C_3}{\varepsilon(1-\beta)}\right)\!+\!1\right)\right)$, and $C_1,\ C_3$ are defined in Theorem \ref{complexity-quantization}.
 \end{corollary}
 %\begin{proof}
 %By solving $\left(\frac{\delta_s'}{\delta_s} +\frac{\delta_w'}{\delta_s\delta_w}\right)\frac{2L\sqrt{G^2+\epsilon d}C_8}{(1-\beta)}\leq \frac{\varepsilon}{2}$, and set $K$ to be the same in both direction, we obtain that when $K \geq \log\left(\frac{8Ld^2\sqrt{G^2+\epsilon d}C_8}{\varepsilon(1-\beta)(1-2^{-m})^2}\right)-m + 1$, this equality always holds. Besides, using theorem \ref{complexity-quantization}, with inequality $\mathbb{E}[\|\nabla f(x_\tau^T)\|^2 \leq \varepsilon/2 +  \left(\frac{\delta_s'}{\delta_s} +\frac{\delta_w'}{\delta_s\delta_w}\right)\frac{2L\sqrt{G^2+\epsilon d}C_8}{(1-\beta)}$, we have $T\geq \frac{16(G^2+\epsilon d)}{(1-\beta)^2\alpha^2 \varepsilon^2}\left(f(x_1)-f^* + C_{11} \right)^2$. Moreover, in each iteration we need to transmit $d(m + \log(\log(G)+K+1))$ bits.
 %By taking $m=1$, we get the desired result.
 %\end{proof}

From the above theorem and corollary,  we can reduce the bits of communication by two-way quantization and error feedback. In addition, the bit communication complexity and iteration complexity are $O(d\log\log \frac{d^3}{\varepsilon})$ and $O(\frac{d^2}{\varepsilon^2})$, respectively. 
Moreover, it can be seen that adding compression in both sides can converge to an arbitrary $\varepsilon$-stationary point when we have large enough communication bandwidth, and sufficient iterations. There is a limited influence when we add quantization into communication if we can have a small additional error $\delta_w'$.  Below, we show that if we replace the quantization mapping in Definition \ref{quantization-mapping-def} as Compressor in Definition \ref{compressor-def} in Algorithms \ref{alg1}-\ref{alg2}, Efficient-Adam can attain the same order of iteration complexity as original Adam without introducing additional error terms. 

\begin{theorem}
\label{compressor-complexity}
% Let $\{x_{t}\}$ be the point generated by Algorithms \ref{alg1}-\ref{alg2} with quantization mapping replaced by compressor as Definition \ref{compressor-def}. Assume that all workers works identically and independently.  In addition, let $x^T_\tau$ be the random variable $x_\tau$ with $\tau$ taking from $\{1,2,\ldots,T\}$ with the same probability. the convergence result holds as follows:  
 %\[
%\mathbb{E}[\|\nabla f(x_\tau^T)\|^2]\leq \frac{1}{\sqrt{T}} \frac{2\sqrt{G^2+\epsilon d}}{\alpha(1-\beta)}(f(x_1) - f^* + C_2),
%\]
Let $\{x_t\}$ be the point generated by Algorithm \ref{alg1} and Algorithm \ref{alg2} with the quantization mapping replaced by the compressor in Definition \ref{compressor-def}. In addition, assume that all workers work identically and independently. Let $x_\tau^T$ be the random variable $x_\tau$ with $\tau$ taking from $\{1,2,\cdots, T\}$ with the same probability. For given $\varepsilon$, when $T\geq \frac{4(G^2+\epsilon d)}{(1-\beta)^2\alpha^2 \varepsilon^2}\left(F(x_1)-F^* + C_{6} \right)^2$, it always holds: 
\[
\mathbb{E}[\|\nabla F(x_\tau^T)\|^2] \leq \varepsilon,
\]
where $C_1 \!=\! \Big(\frac{\beta/(1-\beta)}{\sqrt{(1-\gamma)\theta_1}}+1\Big)^2$, 
and $C_{6} \!=\! \frac{d}{1-\sqrt{\gamma}}\left(\frac{(2-\delta_w)(2-\delta_s)\alpha^2L}{\theta(1-\sqrt{\gamma})^2\delta_w\delta_s} \!+\! \frac{2C_1G\alpha}{\sqrt{\theta}} \right) \left[\log\left(1+\frac{G^2}{\epsilon d}\right)\!+\!\frac{\theta}{1\!-\!\theta}\right]$.
\end{theorem}

From the above theorem, it can be shown that the convergence rate of Efficient-Adam matches the convergence rate of the original Adam. Thanks to the two-way error feedback techniques employed in Efficient-Adam, the convergence rate will not be hurt by the introduced bi-direction compressor as defined in Definition \ref{compressor-def}, which merely affects the speed of convergence at the constant level.

 

==> texfiles/supplementary_compressor.tex <==
\section{Generalized to Compressor}

In this section, we will analyze the converge property of above algorithms. To analyze the converge of the above algorithms we need some more assumptions on quantization functions and hyper-parameter choice.

\begin{assumption}
\label{A2}
For the quantization function used in Algorithm \ref{alg1}, there exists a positive value $\delta_x$, such that the inequality holds: $\|x-Q_x(x)\|\leq (1-\delta_x)\|x\|$.
\end{assumption}

Similarly, we have the addition assumption for the quantization function in Algorithm \ref{alg2}.

\begin{assumption}
\label{A3}
For the quantization function used in Algorithm \ref{alg2}, there exists a positive value $\delta_g$, such that the inequality holds:
$\|x-Q_g(x)\| \leq (1-\delta_g)\|x\|$.
\end{assumption}

In addition, we make the following assumption on momentum average parameter $\beta$, exponential moving average parameter $\theta_t$ and learning rate $\alpha_t$.

\begin{assumption}\label{A4}
We assume that $\theta_t = 1-\frac{\theta}{t}$, and $\alpha_t = \frac{\alpha}{\sqrt{t}}$. Besides, we choose $\theta'$ such that $0<\beta^2<\theta'<1$ and denote $\gamma = \beta/\theta'$. Let $n = max\{j|\theta_j<\theta'\}$, then we denote $C_1 = \prod_{j=1}^n \frac{\theta_j}{\theta'}$.
\end{assumption}

\subsubsection{Single Worker Analysis}
  In this section, we establish the convergence result for single worker. Because there is only one worker, there is not average operation in the algorithm. We can view the composition of 2 quantization functions as one quantization function. For simplicity, we use $Q_g(x)$ to represent the compound function and use $\delta_g$ as the quantization error defined similarly in the Assumption \ref{a3}. 
  
\begin{theorem}
\label{T1}
Let $\{x_t\}$ be the sequence generated by Algorithm \ref{alg1} and Algorithm \ref{alg2}.
In addition, let $x_\tau^T$ represent random variable $x_\tau$ with $\tau$ taking from $\{1,2,\ldots,T\}$ with the same probability. The convergence result holds as follows: 
\begin{equation}
(E[\|\nabla f((x_\tau^T))\|^2]) \leq \frac{C+C'\sum_{t=1}^T\frac{1}{t}}{\sqrt{T}},
\end{equation}
where  $ C_2 = \left(\frac{\beta/(1-\beta)}{\sqrt{C_1(1-\gamma)\theta_1}}+1\right)^2$, $C_3 = \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})} \left(\frac{\alpha L(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_g} + \frac{2C_2G}{\sqrt{\theta}} \right)$, 
    $C = \frac{2\sqrt{G^2+\epsilon d}}{(1-\beta)}\left(f(x_1)-f^*+ \alpha C_3d\log\left(1+\frac{G^2}{\epsilon d}\right)\right)$, and, 
    $C' = \frac{2\sqrt{G^2+\epsilon d}C_3d}{(1-\beta)(1-\theta)}$.
\end{theorem}
The proof of Theorem \ref{T1} can be seen in Section \ref{pft1}. 
From this result, it can be seen that with quantization error will hurt the convergence speed by effect constant $C_3$. This result can reduce to the origin Adam's convergence rate when $\delta_g$ goes to 1, which means no error in quantization. Besides, the order of convergence rate does not hurt by adding quantization, it is still $O(\log(T)/\sqrt{T})$.

\subsubsection{Multi-Worker Analysis}
In this section, we consider multi-worker setting. We denote the number of workers as $N$, and make additional assumption that all workers works identically and independently, i.e. $\xi$ on each worker follows the same distribution and is independent to each other.

\begin{theorem}
\label{T2}
 Let $\{x_{t}\}$ be the point generated by Algorithms \ref{alg1} and Algorithm \ref{alg2}. 
 In addition, let $x^T_\tau$ be the random variable $x_\tau$ with $\tau$ taking from $\{1,2,\ldots,T\}$ with the same probability. the convergence result holds as follows:  
 \[
\mathbb{E}[\|\nabla f(x_\tau)\|^2]\leq \frac{C_5+C_6\sum_{t=1}^T \frac{1}{t}}{\sqrt{T}},
\]
where $C_2 = \left(\frac{\beta/(1-\beta)}{\sqrt{C_1(1-\gamma)\theta_1}}+1\right)^2$,
$C_4 = \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})} \left(\frac{\alpha L(2-\delta_x)(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_x\delta_g} + \frac{2C_2G}{\sqrt{\theta}}\right)$,
$C_5 = \frac{2\sqrt{G^2+\epsilon d}}{\alpha(1-\beta)}\left(f(x_1) - f^* + C_4d\alpha\log\left(1+\frac{G}{\epsilon d}\right)\right),$ and, $C_6 = \frac{2\sqrt{G^2+\epsilon d}C_4 d}{(1-\beta)(1-\theta)}$.

\end{theorem}


The proof of Theorem \ref{T2} is in Section \ref{pft2}. From this result it can be shown that when $delta_x$ goes to 1 or $\delta_g$ goes to 1 the theorem will reduce to Theorem \ref{T1}. And still the convergence rate will not be hurt by adding both direction quantization and quantization error will affect the constant $C_4$ which will effect the speed of convergence in the constant level.



\subsection{Proof of Theorem 1}\label{pft1}
To prove Theorem \ref{T1}, more useful notations and lemmas are needed. So we first introduce some notations in this section. Because there is only one worker, for simplicity, we denote $m_t$, $v_t$ as $m_t^{(1)}$, $v_t^{(1)}$, respectively.notations
\begin{notation}\label{notation-thm1}
Let $\mathbb{E}_t(\cdot) = \mathbb{E}_\xi(\cdot|x_t)$. 
Denote 
$\sigma^2_t = \mathbb{E}_t(g_t^2)$, 
$\hat{v}_t = \theta_t v_t + (1-\theta_t) \sigma^2_t$, 
$\hat{\eta}_t = \alpha_t/\sqrt{\hat{\theta}_t}$, 
$\Delta_t = -\alpha_t m_t/\sqrt{v_t}$, 
$M_t = \mathbb{E}[\langle\nabla f(x_t), \Delta_t\rangle+L(2-\delta_g)\|\Delta_t\|^2 + L(2-\delta_g)\|e_t\|\|\Delta_t\|]$,
 and $\|x\|_{\hat{\eta}_t}^2 = \sum_{i=1}^d \hat{\eta}_t^{(i)}{x^{(i)}}^2$.
In addition, let $\tilde{x}_t = x_t - e_{t}$. Then, it holds that  $\tilde{x}_{t+1} = x_t - Q_g(-\Delta_t+e_t) - e_{t+1} = x_t + \Delta_t -e_t = \tilde{x}_t + \Delta_t$.
\end{notation}

\begin{lemma}\label{Lemmamv}
By using Notation \ref{notation-thm1} and the iteration scheme of Theorem 1, for all $t\ge 1$ the following inequality holds:
\[
  m_t^2\leq \frac{1}{C_1(1-\gamma)(1-\theta_t)}v_t.
\]
\end{lemma}
\begin{proof}
By using the definition of $m_t$ in Theorem 1, it directly holds that
\begin{align}\label{eq-mt}
m_t = \sum_{i=1}^t\beta^{t-i}(1-\beta)g_i.
\end{align}
Let $\Theta(t,i) = \prod_{j=i+1}^t \theta_j$ for $i < t$, and $\Theta(i,i) = 1$. According to the definition of $v_t$, it holds that
\[
   v_t = \sum_{i = 1}^t \left(\prod_{j=i+1}^t\theta_j\right)(1-\theta_i)g_i^2 = \sum_{i = 1}^t\Theta(t,i)(1-\theta_i)g_i^2.
\]
With arithmetic inequality and Eq.~\eqref{eq-mt}, it holds that
\[
\begin{split}
    m_t^2 &= \left(\sum_{i=1}^t\frac{\beta^{t-i}(1-\beta)}{\sqrt{\Theta(t,i)(1-\theta_i)}}\sqrt{\Theta(t,i)(1-\theta_i)}g_i \right)^2
    \leq \sum_{i=1}^t\frac{\beta^{2(t-i)}(1-\beta)^2}{\Theta(t,i)(1-\theta_i)}\sum_{i=1}^t\Theta(t,i)(1-\theta_i)g_i^2\\
    &= \sum_{i=1}^t\frac{\beta^{2(t-i)}(1-\beta)^2}{\Theta(t,i)(1-\theta_i)}v_t
    \leq \sum_{i=1}^t\frac{\beta^{2(t-i)}}{(\prod_{j=i+1}^N\theta_j){\theta'}^{t-N}(1-\theta_i)}v_t
    = \sum_{i=1}^t\frac{\beta^{2(t-i)}}{(\prod_{j=i+1}^N\theta_j/\theta')(\theta')^{t-i}(1-\theta_i)}v_t\\
    &\leq \sum_{i=1}^t\frac{\beta^{2(t-i)}}{(\prod_{j=1}^N\theta_j/\theta')(\theta')^{t-i}(1-\theta_i)}v_t
    = \sum_{i=1}^t\frac{\beta^{2(t-i)}}{C_1(\theta')^{t-i}(1-\theta_i)}v_t
    \leq \frac{1}{C_1(1-\theta_t)}\sum_{i=1}^t \left(\frac{\beta^2}{\theta'}\right)^{t-i}v_t\\
    &\leq \frac{1}{C_1(1-\gamma)(1-\theta_t)}v_t.
\end{split}
\]
Then, we obtain the targeted result. 
\end{proof}



\begin{lemma}\label{ft}
  Let $\tau$ be randomly chosen from $\{1,2,\cdots,T\}$ with equal probabilities $p_\tau = \frac{1}{T}$. We have the following estimate:
  \[
  \mathbb{E}[\|\nabla f((x_\tau))\|^2]\leq \frac{\sqrt{G^2+\epsilon d}}{\alpha\sqrt{T}}\mathbb{E}\left[\sum_{t=1}^T\|\nabla f((x_t))\|_{\hat{\eta_t}}^2\right].
  \]
\end{lemma}
\begin{proof}
Note that $\|\hat{v}_t\|_1 = \theta_t \|v_{t-1}\|_1 +(1-\theta_t) \|\sigma_t\|^2$ and $\|g_t\|\leq G$. It is straightforward to prove $\|v_t\|_1 \leq G^2$. Hence, we have $\|\hat{v}_t + \epsilon\|_1 \leq G^2 + \epsilon d$. Utilizing this inequality, we have
\[
\begin{split}
     \|\nabla f(x_t)\|^2 &= \frac{\|\nabla f(x_t)\|^2}{\sqrt{\|\hat{v}_t+\epsilon\|_1}}\sqrt{\|\hat{v}_t+\epsilon\|_1} = \sqrt{\|\hat{v}_t +\epsilon \|_1}\sum_{k=1}^d\frac{|\nabla_k f(x_t)|^2}{\sqrt{\sum_{l=1}^d \hat{v}_{t,l}+\epsilon}}\\
     &\leq \sqrt{\|\hat{v}_t+\epsilon\|_1}\alpha_t^{-1}\sum_{k=1}^d \frac{\alpha_t}{\sqrt{\hat{v}_{t,k}+\epsilon}}|\nabla_k f(x_t)|^2 \\
     &= \sqrt{\|\hat{v}_t+\epsilon\|_1}\alpha_t^{-1}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2 \leq \sqrt{G^2+\epsilon d}\alpha_t^{-1}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2\\
     &\leq \frac{\sqrt{G^2 + \epsilon d}}{\alpha_T}\|\nabla f(x_t)\|^2_{\hat{\eta}_t}.
\end{split}
\]
Then, by using the definition of $x_{\tau}$, we obtain
\[
     \mathbb{E}\left[\|\nabla f(x_\tau)\|^2\right] = \frac{1}{T}\sum_{t=1}^T\mathbb{E}\left[\|\nabla f(x_t)\|^2\right] \leq \frac{\sqrt{G^2 + \epsilon d}}{\alpha\sqrt{T}} \mathbb{E}\left[\sum_{t=1}^T \|\nabla f(x_t)\|^2_{\hat{\eta}_t}\right].
\]
Thus, the desired result is obtained. 
\end{proof}

\begin{lemma}\label{sumdelta}
By using Notation\ref{notation-thm1}, the following inequality holds:
\[
\sum_{i=1}^T \|\Delta_t\|^2 \leq \frac{\alpha^2}{C_1\theta(1-\sqrt{\gamma})^2}\sum_{t=1}^T\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2
\]
\end{lemma}
\begin{proof}
By the definition of $m_t$, we can obtain
\[
|m_t| = \left|\sum_{i=1}^t \beta^{t-i}(1-\beta)g_i\right|\leq \sum_{i=1}^t \beta^{t-i}|g_i|.
\]

Because $v_t \geq \theta_t v_{t-1}$, we can easily obtain that $v_t \geq \Theta(t,i) v_i$, where $\Theta(t,i)$ is defined in Lemma \ref{Lemmamv}.

Besides, by using the definition of $\theta'$ in Assumption \ref{A4}, we can obtain
\[
\Theta(t,i) = \prod_{j=i+1}^t \theta_j  \geq (\theta')^{t-n}\prod_{j=i+1}^n \theta_j =(\theta')^{t-i}\prod_{j=i+1}^n (\theta_j/\theta') \geq (\theta')^{t-i}\prod_{j=1}^n (\theta_j/\theta') = C_1 \theta'^{t-i}.
\]

Therefore, we obtain $v_t\geq C_1(\theta')^{t-i}v_i$.

By using the definition of $\Delta_t$, we can obtain
\[
\begin{split}
\|\Delta_t\|^2 &= \left\|\frac{\alpha_t m_t}{\sqrt{v_t}}\right\|^2 \leq \alpha_t^2 \sum_{i=1}^t \left\|\frac{\beta^{t-i}|g_i|}{\sqrt{v_t}}\right\|^2\leq \frac{\alpha_t^2}{(1-\theta_t)C_1} \sum_{i=1}^t\left\|\left(\frac{\beta}{\sqrt{\theta'}}\right)^{t-i} \frac{\sqrt{1-\theta_t} |g_i|}{\sqrt{v_t}}\right\|^2\\
&\leq \frac{\alpha^2}{C_1\theta}\sum_{i=1}^t\left\|\sqrt{\gamma}^{t-i}\frac{\sqrt{1-\theta_i}|g_i|}{\sqrt{v_i}}\right\|^2 \leq \frac{\alpha^2}{C_1\theta}(\sum_{i=1}^t\sqrt{\gamma}^{t-i})\sum_{i=1}^t \sqrt{\gamma}^{t-i}\left\|\frac{\sqrt{1-\theta_i}g_i}{\sqrt{v_i}}\right\|^2\\
&\leq \frac{\alpha^2}{C_1\theta(1-\sqrt{\gamma})}\sum_{i=1}^t \sqrt{\gamma}^{t-i}\left\|\frac{\sqrt{1-\theta_i}g_i}{\sqrt{v_i}}\right\|^2
\end{split}
\]

Hence, it follows that
\[
\begin{split}
\sum_{t=1}^T\|\Delta_t\|^2 &\leq \frac{\alpha^2}{C_1\theta(1-\sqrt{\gamma})}\sum_{t=1}^T\sum_{i=1}^t \sqrt{\gamma}^{t-i}\left\|\frac{\sqrt{1-\theta_i}g_i}{\sqrt{v_i}}\right\|^2 \\
& = \frac{\alpha^2}{C_1\theta(1-\sqrt{\gamma})}\sum_{i=1}^T \sum_{t=i}^T \sqrt{\gamma}^{t-i} \left\|\frac{\sqrt{1-\theta_i}g_i}{\sqrt{v_i}}\right\|^2\\
&\leq \frac{\alpha^2}{C_1\theta(1-\sqrt{\gamma})^2}\sum_{t=1}^T \left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2
\end{split}
\]
Thus, the desired result is obtained.
\end{proof}


\begin{lemma}\label{matrix}
By the iteration scheme of Algorithm 1, it holds that
\[
\sum_{t = 1}^T \|e_t\|\|\Delta_t\| \leq \sum_{t=1}^T\frac{1-\delta_g}{\delta_g} \|\Delta_t\|^2.
\]
\end{lemma}
\begin{proof}
By the definition of noisy term $e_{t}$ and $\Delta_{t}$, it holds
\[
\begin{split}
  \|e_t\|  &= \|\Delta_{t-1} + e_{t-1} - Q_g(\Delta_{t-1} + e_{t-1}) \| \leq (1-\delta_g) \|\Delta_{t-1} + e _{t-1}\|\leq (1-\delta_g) \|\Delta_{t-1}\| + (1-\delta_g)\|e_{t-1}\|\\
  &\leq \sum_{i=1}^{t-1} (1-\delta_g)^{t-i}\|\Delta_i\|.
\end{split}
\]
Therefore, we have 
\begin{align}\label{cross-noisy-eq}
    \sum_{t = 1}^T \|e_t\|\|\Delta_t\| \leq \sum_{t=1}^T\sum_{i=1}^{t-1} (1-\delta_g)^{t-i}\|\Delta_i\|\|\Delta_t\|.
\end{align}
In addition, let $\Delta = \left[ \begin{array}{cccc}\|\Delta_1\|&\|\Delta_2\|&\cdots&\|\Delta_T\|\end{array}\right]^{\top}$ and $U$ be the following $T\times T$ matrix:
\[
U = \left [ 
\begin{array}{ccccc}
0& (1-\delta_g)/2 & (1-\delta_g)^2/2 &\cdots&(1-\delta_g)^{T-1}/2\\
(1-\delta_g)/2 & 0& (1-\delta_g)/2 &\cdots&(1-\delta_g)^{T-2}/2\\
(1-\delta_g)^2/2 & (1-\delta_g)/2 & 0 &\cdots&(1-\delta_g)^{T-3}/2\\
\vdots&\vdots&\vdots&\ddots&\vdots\\
(1-\delta_g)^{T-1}/2 & (1-\delta_g)^{T-2}/2 & (1-\delta_g)^{T-3}/2 &\cdots&0
\end{array}\right].
\]
Let $\rho(U)$ be the spectral radius of $U$ and $\|U\|_{\infty}$ be $\infty$-norm which is defined to be the maximal row sum of $U$. Then, it holds that
\[
  \rho(U) \leq \|U\|_{\infty} \leq 2\sum_{t=1}^{T/2+1} (1-\delta_g)^t/2 \leq \frac{1-\delta_g}{\delta_g}.
\]
Utilizing the above inequality, we obtain 
\[
     \sum_{t=1}^T\sum_{i=1}^t (1-\delta_g)^{t-i+1}\|\Delta_i\|\|\Delta_t\| = \Delta^TU\Delta \leq \rho(U)\Delta^T\Delta \leq  \frac{1-\delta_g}{\delta_g} \sum_{t=1}^T\|\Delta_t\|^2.
\]
Substituting the above inequality into Eq.~\eqref{cross-noisy-eq}, we obtain the desired result.
\end{proof}

\begin{lemma}\label{sumgv}
The following estimate holds:
\[
\mathbb{E}\left[\sum_{t=1}^T\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2\right] \leq d\left[\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right].
\]
\end{lemma}

\begin{proof}
Let $W_0 = 1$ and $W_t = \prod_{i=1}^t \theta_i^{-1}$. Let $w_t = W_t-W_{t-1} = (1-\theta_t)W_t$. 

Therefore, we have $\frac{w_t}{W_t} = 1-\theta_t$, and $\frac{W_{t-1}}{W_t} = \theta_t$.

By observing that $W_0v_0 = \epsilon$ and $W_tv_t = W_{t-1}v_{t-1} + w_t g_t^2$, then we can obtain 
\[W_tv_t = \epsilon + \sum_{i=1}^tw_ig_i^2\].

By plugging the equality into the left hand side, we obtain
\[
\begin{split}
\sum_{t=1}^T\left\|\frac{\sqrt{1-\theta_t} g_t}{\sqrt{v_t}}\right\|^2 &= \sum_{t=1}^T \left\|\frac{(1-\theta_t)g_t^2}{v_t}\right\|_1 = \sum_{t=1}^T \left\|\frac{w_tg_t^2}{W_tv_t}\right\|_1 = \sum_{t=1}^T\left\|\frac{w_tg_t^2}{\epsilon + \sum_{i=1}^t w_ig_i^2}\right\|_1\\
& =\sum_{t=1}^T\sum_{k=1}^d \frac{w_tg_{t,k}^2}{\epsilon+\sum_{i=1}^t w_ig_{i,k}^2} = \sum_{k=1}^d\sum_{t=1}^T \frac{w_tg_{t,k}^2}{\epsilon+\sum_{i=1}^t w_ig_{i,k}^2}.
\end{split}
\] 

Considering each dimension respectively, for each $k=1,2,\cdots,d$, we obtain
\[
 \sum_{t=1}^T \frac{w_tg_{t,k}^2}{\epsilon+\sum_{i=1}^t w_ig_{i,k}^2} \leq \log\left(\epsilon + \sum_{i=1}^tw_ig_{i,k}^2\right) - \log(\epsilon) = \log\left(1 + \frac{1}{\epsilon}\sum_{i=1}^tw_ig_{i,k}^2\right).
\]

Therefore, 
\[
\begin{split}
\sum_{t=1}^T\left\|\frac{\sqrt{1-\theta_t} g_t}{\sqrt{v_t}}\right\|^2 &\leq \sum_{k=1}^d \log\left(1 + \frac{1}{\epsilon}\sum_{i=1}^Tw_ig_{i,k}^2\right) \leq  d\log\left(1 + \frac{1}{d\epsilon}\sum_{k=1}^d \sum_{i=1}^Tw_ig_{i,k}^2\right)\\
&= d\log\left(1 + \frac{1}{d\epsilon}\sum_{i=1}^Tw_i\|g_i\|^2\right) \leq d\log\left(1 + \frac{G^2}{d\epsilon}(W_T-W_0)\right)\\
&=d\log\left(1 + \frac{G^2}{d\epsilon}\left(\prod_{i=1}^T \theta_i^{-1} -1\right)\right) \leq d\left[\log\left(1+\frac{G^2}{d\epsilon}\right) + \sum_{t=1}^T\log(\theta_t^{-1})\right]\\
&\leq d\left[\log\left(1+\frac{G^2}{d\epsilon}\right) + \sum_{t=1}^T \left(\theta_t^{-1} -1\right)\right] \leq d\left[\log\left(1+\frac{G^2}{d\epsilon}\right) + \frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right].
\end{split}
\]

Hence, we obtain desired result.
\end{proof}

\begin{lemma}\label{Mt}
By the definition of $M_t$, it holds that 
\[
\sum_{t=1}^T M_t \leq C_3d\alpha\left(\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right)- \frac{1-\beta}{2}\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2,
\]
where 
\[
\begin{split}
C_2 &= \left(\frac{\beta/(1-\beta)}{\sqrt{C_1(1-\gamma)\theta_1}}+1\right)^2\\
C_3 &= \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})} \left(\frac{\alpha L(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_g} + \frac{2C_2G}{\sqrt{\theta}} \right) 
\end{split}
\]
\end{lemma}
\begin{proof}
Using the definitions of $v_t$ and $\hat{v}_t$, we obtain
\[
\begin{split}
\frac{(1-\beta)\alpha_tg_t}{\sqrt{v_t}} &= \frac{(1-\beta)\alpha_tg_t}{\sqrt{\hat{v}_t}} + (1-\beta)\alpha_tg_t\left(\frac{1}{\sqrt{v_t}} - \frac{1}{\sqrt{\hat{v}_t}}\right)\\
&= (1-\beta)\hat{\eta}_tg_t + (1-\beta)\alpha_tg_t\frac{(1-\theta_t)(\sigma_t^2-g_t^2)}{\sqrt{v_t}\sqrt{\hat{v}_t}(\sqrt{v_t}+\sqrt{\hat{v}_t})}\\
&= (1-\beta)\hat{\eta}_tg_t+ \hat{\eta}_t\sigma_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}\frac{(1-\beta)\sigma_t}{\sqrt{v_t}+\sqrt{\hat{v}_t}} - \hat{\eta}_tg_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}\frac{(1-\beta)g_t}{\sqrt{v_t}+\sqrt{\hat{v}_t}}.
\end{split}
\]

In addition, we can obtain that
\[
\begin{split}
&\beta\alpha_tm_{t-1}\left(\frac{1}{\sqrt{v_t}} - \frac{1}{\sqrt{\theta_tv_{t-1}}}\right) = \beta\alpha_tm_{t-1}\frac{(1-\theta_t)g_t^2}{\sqrt{v_t}\sqrt{\theta_tv_{t-1}}(\sqrt{v_t}+\sqrt{\theta_tv_{t-1}})}\\
&\qquad =\beta\alpha_tm_{t-1}\frac{(1-\theta_t)g_t^2}{\sqrt{v_t}+\sqrt{\theta_tv_{t-1}}} + \beta\alpha_tm_{t-1} \frac{(1-\theta_t)g_t^2}{\sqrt{v_t}(\sqrt{v_t} + \sqrt{\theta_tv_{t-1}})} \left(\frac{1}{\sqrt{\theta_tv_{t-1}}} - \frac{1}{\sqrt{\hat{v}_t}}\right)\\
&\qquad = \hat{\eta}_tg_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}\left(\frac{\beta m_{t-1}}{\sqrt{v_t} +\sqrt{\theta_t v_{t-1}}}\right) + \frac{\beta\alpha_t m_{t-1}(1-\theta_t)g_t^2\sigma_t^2}{\sqrt{v_t}\sqrt{\hat{v}_t}\sqrt{\theta_tv_{t-1}}(\sqrt{v_t}+\sqrt{\theta_tv_{t-1}})(\sqrt{\hat{v}_t}+\sqrt{\theta_tv_{t-1}})}\\
& \qquad = \hat{\eta}_tg_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}\left(\frac{\beta m_{t-1}}{\sqrt{v_t} +\sqrt{\theta_t v_{t-1}}}\right) + \hat{\eta}_t\sigma_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}\left(\frac{\beta m_{t-1}}{\sqrt{\theta_tv_{t-1}}} \frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}+\sqrt{\theta_tv_{t-1}}} \frac{\sqrt{1-\theta_t}\sigma_t}{\sqrt{\hat{v}_t}+\sqrt{\theta_tv_{t-1}}} \right).
\end{split}
\]

For convenience, we denote
\[
\begin{split}
A_t &= \frac{\beta m_{t-1}}{\sqrt{v_t} + \sqrt{\theta_t v_{t-1}}} - \frac{(1-\beta)g_t}{\sqrt{v_t} + \sqrt{\hat{v}_t}},\\
B_t &= \left(\frac{\beta m_{t-1}}{\sqrt{\theta_tv_{t-1}}} \frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}+\sqrt{\theta_tv_{t-1}}} \frac{\sqrt{1-\theta_t}\sigma_t}{\sqrt{\hat{v}_t}+\sqrt{\theta_tv_{t-1}}} \right) +\frac{(1-\beta)\sigma_t}{\sqrt{v}_t +\sqrt{\hat{v}_t}}.
\end{split}
\]

Then, for each $t>2$, we obtain
\[
\begin{split}
\Delta_t - \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}\Delta_{t-1} &= -\frac{\alpha_tm_t}{\sqrt{v_t}} + \frac{\beta\alpha_tm_{t-1}}{\sqrt{\theta_tv_{t-1}}} = -\alpha_t\left(\frac{m_t}{\sqrt{v_t}} - \frac{\beta m_{t-1}}{\sqrt{\theta_tv_{t-1}}}\right)\\
& = -\frac{(1-\beta)\alpha_tg_t}{\sqrt{v_t}} - \beta\alpha_tm_{t-1}\left(\frac{1}{\sqrt{v_t}} - \frac{1}{\sqrt{\theta_tv_{t-1}}}\right)\\
& = -(1-\beta)\hat{\eta}_tg_t - \hat{\eta}_tg_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}A_t - \hat{\eta}_t\sigma_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}B_t. 
\end{split}
\]

By using the above equality, we can get an upper bound for  $\mathbb{E}\langle \nabla f(x_t), \Delta_t\rangle$:
\[
\begin{split}
\mathbb{E} \langle \nabla f(x_t),\Delta_t \rangle &= \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}\mathbb{E}\langle \nabla f(x_t),\Delta_{t-1}\rangle + \mathbb{E} \left\langle \nabla f(x_t),\Delta_t - \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}\Delta_{t-1}\right\rangle\\
& = \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}\mathbb{E}\langle \nabla f(x_t),\Delta_{t-1}\rangle - \mathbb{E} \left\langle \nabla f(x_t),(1-\beta)\hat{\eta}_tg_t\right\rangle \\
&\qquad - \mathbb{E}\left \langle \nabla f(x_t), \hat{\eta}_tg_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}A_t\right\rangle -\mathbb{E}\left\langle \nabla f(x_t), \hat{\eta}_t\sigma_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}B_t \right\rangle.
\end{split}
\]

We split $\mathbb{E}\langle \nabla f(x_t), \Delta_t\rangle$ into 4 terms, and we analyze these 4 terms respectively. For the first term, we obtain
\[
\begin{split}
\frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}\mathbb{E}\langle \nabla f(x_t),\Delta_{t-1}\rangle &= \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}\mathbb{E}\left(\langle \nabla f(x_{t-1}), \Delta_{t-1}\rangle + \langle \nabla f(x_t) - \nabla f(x_{t-1}), \Delta_{t-1}\rangle \right)\\
&\leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}} \mathbb{E} (\langle \nabla f(x_{t-1}), \Delta_{t-1}\rangle + L\|x_t - x_{t-1}\|\|\Delta_{t-1}\|)\\
&\leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}} \mathbb{E} (\langle \nabla f(x_{t-1}), \Delta_{t-1}\rangle + L\|Q_g(\Delta_{t-1}+e_{t-1})\|\|\Delta_{t-1}\|)\\
&\leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}} \mathbb{E} (\langle \nabla f(x_{t-1}), \Delta_{t-1}\rangle\\ &\qquad + L\|Q_g(\Delta_{t-1}+e_{t-1}) - (\Delta_{t-1}+e_{t-1}) + (\Delta_{t-1}+e_{t-1})\|\|\Delta_{t-1}\|)\\
&\leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}} \mathbb{E} (\langle \nabla f(x_{t-1}), \Delta_{t-1}\rangle\\ &\qquad + L((1-\delta_g)\|\Delta_{t-1}+e_{t-1}\| + \|\Delta_{t-1}+e_{t-1}\|)\|\Delta_{t-1}\|)\\
&\leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}} \mathbb{E} (\langle \nabla f(x_{t-1}), \Delta_{t-1}\rangle + L(2-\delta_g)\|\Delta_{t-1}+e_{t-1}\|\|\Delta_{t-1}\|)\\
&\leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}} \mathbb{E} (\langle \nabla f(x_{t-1}), \Delta_{t-1}\rangle + L(2-\delta_g)\|\Delta_{t-1}\|^2+ L(2-\delta_g)\|e_{t-1}\|\|\Delta_{t-1}\|)\\
&= \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}} M_{t-1}.
\end{split}
\]

For the second term, we have
\[
-\mathbb{E}\langle\nabla f(x_t), (1-\beta)\hat{\eta}_tg_t\rangle = -(1-\beta) \mathbb{E}\langle \nabla f(x_t), \hat{\eta_t}\mathbb{E}_t(g_t)\rangle = -(1-\beta)\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2.
\]

For the third term, we have 
\[
\begin{split}
-\mathbb{E}\left\langle \nabla f(x_t), \hat{\eta}_tg_t \frac{(1-\theta_t)g_t}{\sqrt{v_t}} A_t \right\rangle &\leq \mathbb{E} \left\langle \frac{\sqrt{\hat{\eta}_t}|\nabla f(x_t)||g_t|}{\sigma_t}, \frac{\sqrt{\hat{\eta}_t}\sigma_t|A_t|(1-\theta_t)|g_t|}{\sqrt{v_t}}\right\rangle\\
&\leq \frac{1-\beta}{4}\mathbb{E}\left\|\frac{\sqrt{\hat{\eta}_t}|\nabla f(x_t)||g_t|}{\sigma_t}\right\|^2 + \frac{1}{1-\beta}\mathbb{E}\left\|\frac{\sqrt{\hat{\eta}_t}\sigma_t|A_t|(1-\theta_t)|g_t|}{\sqrt{v_t}}\right\|^2\\
&\leq \frac{1-\beta}{4}\mathbb{E}\|\nabla f(x_t)\|^2_{\hat{\eta}_t} + \frac{C_2G\alpha}{\theta}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2.
\end{split}
\]
where the inequality holds with the following equalities and inequalities:
\[
\mathbb{E}\left\|\frac{\sqrt{\hat{\eta}_t}|\nabla f(x_t)||g_t|}{\sigma_t}\right\|^2 = \mathbb{E}\left\|\frac{\hat{\eta}_t\nabla f(x_t)^2g_t^2}{\sigma_t^2}\right\|_1 = \mathbb{E} \|\hat{\eta}_t\nabla f(x_t)^2\|_1 = \mathbb{E}\|\nabla f(x_t)\|^2_{\hat{\eta}_t},
\]
\[
\sqrt{\hat{\eta}_t}\sigma_t \leq \sqrt{\frac{\alpha_t\sigma_t^2}{\sqrt{(1-\theta_t)\sigma_t^2}}} \leq \sqrt{\frac{\alpha G}{\sqrt{\theta}}},
\]
and 
\[
\begin{split}
|A_t| &\leq \frac{\beta|m_{t-1}|}{\sqrt{\theta_t v_{t-1}}} + \frac{(1-\beta)|g_t|}{\sqrt{v_t}} \leq  \frac{\beta}{\sqrt{\theta_tC_1(1-\gamma)(1-\theta_t)}} + \frac{1-\beta}{\sqrt{1-\theta_t}}.
\end{split}
\]

Let $C_2 = \left(\frac{\beta/(1-\beta)}{\sqrt{C_1(1-\gamma)\theta_1}}+1\right)^2$, we can obtain $|A_t|\leq \frac{\sqrt{C_2}(1-\beta)}{\sqrt{1-\theta_t}}$.

Then we obtain the upper bound of the third term.

For the fourth term, by using the similar inequalities we have
\[
|B_t| \leq \left(\frac{\beta|m_{t-1}|}{\sqrt{\theta_tv_{t-1}}} \frac{\sqrt{1-\theta_t}|g_t|}{\sqrt{v_t}+\sqrt{\theta_t v_t}}\frac{\sqrt{1-\theta_t}\sigma_t}{\sqrt{\hat{v}_t}+\sqrt{\theta_t v_{t-1}}}\right) + \frac{(1-\beta)\sigma_t}{\sqrt{v_t}+\sqrt{\hat{v}_t}} \leq \frac{(1-\beta)\sqrt{C_2}}{\sqrt{1-\theta_t}}.
\]

Then, the fourth term will be bounded as follows:
\[
\begin{split}
-\mathbb{E}\left\langle \nabla f(x_t), \hat{\eta}_t\sigma_t\frac{(1-\theta_t)g_t}{\sqrt{v_t}}B_t \right\rangle &\leq \mathbb{E}\left\langle \sqrt{\hat{\eta}}_t |\nabla f(x_t)|, \frac{\sqrt{\hat{\eta}_t}\sigma_t|B_t|(1-\theta_t)|g_t|}{\sqrt{v_t}}\right\rangle\\
&\leq \mathbb{E}\left\langle \sqrt{\hat{\eta}}_t |\nabla f(x_t)|, \frac{\frac{\sqrt{GC_2\alpha}}{\sqrt{\sqrt{\theta}}}\sqrt{1-\theta_t}|g_t|}{\sqrt{v_t}}\right\rangle\\
&\leq \frac{1-\beta}{4} \mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2 + \frac{C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2
\end{split}
\]

Combining the above four terms, we obtain that
\[
\mathbb{E}\langle f(x_t),\Delta_t\rangle \leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}M_{t-1} + \frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2 - \frac{1-\beta}{2}\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2
\]

On the other hand, Let $N_t = L(2-\delta_g)\mathbb{E}\|\Delta_t\|^2 + L(2-\delta_g)\mathbb{E}\|e_t\|\|\Delta_t\| + \frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2$, then with induction we can find the upper bound for $M_t$.  With the above bound, we have 
\[
M_t\leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}M_{t-1}+ N_t - \frac{1-\beta}{2}\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2 \leq \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}M_{t-1}+ N_t.
\] 

Besides, for $M_1$, we have
\[
\begin{split}
  M_1 &= \mathbb{E}\left\langle \nabla f(x_1), -\frac{\alpha_1 m_1}{\sqrt{v_1}}\right\rangle + L(2-\delta_g)\mathbb{E}\|\Delta_1\|^2 + L(2-\delta_g)\mathbb{E}\|e_1\|\|\Delta_1\|\\
  & = -\mathbb{E}\left\langle \nabla f(x_1), \frac{\alpha_1 (1-\beta)g_1}{\sqrt{v_1}}\right\rangle + L(2-\delta_g)\mathbb{E}\|\Delta_1\|^2 + L(2-\delta_g)\mathbb{E}\|e_1\|\|\Delta_1\|\\
  &= -\mathbb{E}\langle \nabla f(x_t), (1-\beta)\hat{\eta}_1g_1\rangle + \mathbb{E}\left\langle \nabla f(x_t), \hat{\eta}_1\sigma_1\frac{(1-\theta_1)g_1}{\sqrt{v_1}}\frac{(1-\beta)\sigma_1}{\sqrt{v_1}+\sqrt{\hat{v}_1}}\right\rangle \\
  & \qquad - \mathbb{E}\left\langle \nabla f(x_t), \hat{\eta}_1g_1\frac{(1-\theta_1)g_1}{\sqrt{v_1}}\frac{(1-\beta)g_1}{\sqrt{v_1}+\sqrt{\hat{v}_1}} \right\rangle + L(2-\delta_g)\mathbb{E}\|\Delta_1\|^2 + L(2-\delta_g)\mathbb{E}\|e_1\|\|\Delta_1\|\\
  &\leq \frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_1}g_1}{\sqrt{v_1}}\right\|^2 - \frac{1-\beta}{2}\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2 + L(2-\delta_g)\mathbb{E}\|\Delta_1\|^2 + L(2-\delta_g)\mathbb{E}\|e_1\|\|\Delta_1\|\\
  &\leq N_1. 
  \end{split}
\]

Therefore, we can obtain
\[
\begin{split}
M_t \leq \sum_{i=1}^t \frac{\alpha_t\beta^{t-i}}{\alpha_i\sqrt{\Theta(t,i)}}N_i - \frac{1-\beta}{2}\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2 \leq \frac{1}{\sqrt{C_1}} \sum_{i=1}^t \sqrt{\gamma}^{t-i}N_i - \frac{1-\beta}{2}\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2,
\end{split}
\]
where the last inequality is because $\alpha_t\leq \alpha_i$ and $\Theta(t,i)\geq C_1 (\theta')^{t-i}$.

Then, by summing $M_t$ up, we obtain
\[
\begin{split}
\sum_{t=1}^T M_t &\leq \frac{1}{\sqrt{C_1}}\sum_{t=1}^T\sum_{i=1}^t\sqrt{\gamma}^{t-i} N_i - \frac{1-\beta}{2}\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2\\
& = \frac{1}{\sqrt{C_1}}\sum_{i=1}^T\sum_{t=i}^T\sqrt{\gamma}^{t-i} N_i - \frac{1-\beta}{2}\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2\\
&\leq \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})}\sum_{t=1}^T N_t - \frac{1-\beta}{2}\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2.
\end{split}
\]

Meanwhile, we can bound summation of $N_t$ by the following terms:
\[
\begin{split}
\sum_{t=1}^T N_t &= \sum_{t=1}^T L(2-\delta_g)\mathbb{E}\|\Delta_t\|^2 + L(2-\delta_g)\mathbb{E}\|e_t\|\|\Delta_t\| + \frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2\\
&\leq \sum_{t=1}^T \frac{L(2-\delta_g)}{\delta_g}\mathbb{E}\|\Delta_t\|^2 + \frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2\\
&\leq \sum_{t=1}^T\left(\frac{\alpha^2L(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_g} + \frac{2C_2G\alpha}{\sqrt{\theta}} \right)\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t}{\sqrt{v_t}}\right\|^2\\
&\leq \left(\frac{\alpha^2L(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_g} + \frac{2C_2G\alpha}{\sqrt{\theta}} \right) d\left[\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right].
\end{split}
\]
Thus, by combining those inequalities we obtain the desired result.
\end{proof}


\begin{proof}[Proof of Theorem 1]
 Based on Notation \eqref{notation-thm1} and the above lemmas, then we can prove Theorem 1. First, according to the gradient Lipschitz condition of $f$, it holds
\[
\begin{split}
f(\tilde{x}_{t+1}) &\leq f(\tilde{x}_t) + \langle\nabla f(\tilde{x}_t), \Delta_t\rangle + \frac{L}{2} \|\Delta_t^2\|\\
& =  f(\tilde{x}_t) + \langle\nabla f(x_t), \Delta_t\rangle + \frac{L}{2} \|\Delta_t\|^2 +\langle\nabla f(\tilde{x}_t)  - \nabla f(x_t), \Delta_t\rangle\\
&\leq  f(\tilde{x}_t) + \langle\nabla f(x_t), \Delta_t\rangle + \frac{L}{2} \|\Delta_t\|^2 + \|\nabla f(\tilde{x}_t) - \nabla f(x_t)\|\|\Delta_t\|\\
&\leq f(\tilde{x}_t) + \langle\nabla f(x_t), \Delta_t\rangle +  L(2-\delta_g)\|\Delta_t\|^2 + L(2-\delta_g)\|e_t\|\|\Delta_t\|.
\end{split}
\]
Recall that $M_t = \mathbb{E}[\langle\nabla f(x_t), \Delta_t\rangle+L(2-\delta_g)\|\Delta_t\|^2 + L(2-\delta_g)\|e_t\|\|\Delta_t\|]$. 
Then we have
\[
\begin{split}
    f^*&\leq \mathbb{E}[f(\tilde{x}_{T+1})] \leq f(x_1) + \sum_{t=1}^T M_t\\
    & \leq f(x_1) + \sum_{t=1}^T M_t\leq f(x_1) + C_3d\alpha\left(\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right)- \frac{1-\beta}{2}\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t}^2.\\
\end{split}
\]
Using the above lemmas and arranging the corresponding terms, we have
\[
\begin{split}
    (\mathbb{E}[\|\nabla f((x_\tau^T))\|^2]) &\leq \frac{\sqrt{G^2+\epsilon d}}{\alpha\sqrt{T}}\mathbb{E}\left[\sum_{t=1}^T\|\nabla f(x_t)\|_{\hat{\eta}_t}^2\right]\\&\leq \frac{2\sqrt{G^2+\epsilon d}}{(1-\beta)\alpha\sqrt{T}}\left(f(x_1) - f^* + C_3d\alpha\left(\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right)\right)\\
    & \leq \frac{C+C'\sum_{t=1}^T\frac{1}{t}}{\sqrt{T}},
\end{split}
\]
where $C_3$, $C'$ and $C'$ are defined as follows,
\[
\begin{split}
    C_2 &= \left(\frac{\beta/(1-\beta)}{\sqrt{C_1(1-\gamma)\theta_1}}+1\right)^2,\\
    C_3 &= \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})} \left(\frac{\alpha L(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_g} + \frac{2C_2G}{\sqrt{\theta}} \right),\\ 
    C &= \frac{2\sqrt{G^2+\epsilon d}}{(1-\beta)\alpha}\left(f(x_1)-f^*+ \alpha C_3d\log\left(1+\frac{G^2}{\epsilon d}\right)\right),\\
    C'& = \frac{2\sqrt{G^2+\epsilon d}C_3d}{(1-\beta)(1-\theta)},
\end{split}
\]
respectively. Hence, the proof is completed.
\end{proof}



\subsection{Proof of Theorem 2}\label{pft2}
To prove Theorem 2, we still need some useful lemmas and notations as follows:
\begin{notation}\label{notation-thm2}
Let $\mathbb{E}_t(\cdot) = \mathbb{E}_\xi(\cdot|x_t)$. 
Denote 
${\sigma^{(i)}_t}^2 = \mathbb{E}_t(g_t^2)$, 
$\hat{v}^{(i)}_t = \theta_t v^{(i)}_t + (1-\theta_t) {\sigma^{(i)}}^2_t$, 
$\hat{\eta}^{(i)}_t = \alpha_t/\sqrt{\hat{\theta}^{(i)}_t}$, 
$\Delta_t^{(i)} = -\alpha_t m_t^{(i)}/\sqrt{v_t^{(i)}}$,
$\Delta_t = \frac{1}{N}\sum_{i=1}^N \Delta_t^{(i)}$, 
$E_t = \frac{1}{N}\sum_{i=1}^N e_t^{(i)}$, and,
$M_t = \mathbb{E}[\langle \nabla f(x_{t}),\Delta_{t}\rangle + \frac{L(2-\delta_x)}{N}\sum_{i=1}^N \|e_{t}\|\|\Delta_{t}^{(i)}\| + \frac{L(2-\delta_x)(2-\delta_g)}{N}\sum_{i=1}^N \|\Delta_{t}^{(i)}\|^2 $ $+ \frac{L(2-\delta_x)(2-\delta_g)}{N^2}\sum_{i=1}^N\sum_{j=1}^N\|e_{t}^{(i)}\|\|\Delta_{t}^{(j)}\|]$.

In addition, let $\tilde{x}_t = x_t - e_{t}$, and,  $ \hat{x_t} = \tilde{x}_t - E_t$. 

Then, it holds that  $\tilde{x}_{t+1} = x_t - Q_x(\hat{\delta}_t+e_t) - e_{t+1} = x_t + \hat{\delta}_t -e_t = \tilde{x}_t + \hat{\delta}_t$.

Besides, $\hat{x}_{t+1} = \tilde{x_t} - \frac{1}{N}\sum_{t=1}^N Q_g(-\Delta_t^{(i)} +e_t^{(i)}) - E_{t+1} = \tilde{x_t} - \frac{1}{N}\sum_{t=1}^N -\Delta_t^{(i)} - E_{t} = \hat{x}_t + \Delta_t$.
\end{notation}



\begin{lemma}
Let $e^{(i)}_t$ be the noisy term defined in Algorithm \ref{alg2} and $\Delta^{(i)}_t$ be the term defined in Notation \ref{notation-thm2}. Then it holds that 
\[
\mathbb{E}\left[\frac{1}{N^2}\sum_{t=1}^T\sum_{i=1}^N\sum_{j=1}^N \|e_t^{(i)}\|\|\Delta_t^{(j)}\|\right] \leq \frac{1-\delta_g}{\delta_gN}\sum_{i=1}^N \mathbb{E}\left[\sum_{t=1}^T\|\Delta_t^{(i)}\|^2\right].
\]
\end{lemma}
\begin{proof}
Using the definition of the noisy term  $e_{t}$, the following holds:
\[
    \|e^{(j)}_t\| = \|\Delta_{t-1}^{(j)} + e_{t-1}^{(j)} - Q_g(\Delta_{t-1}^{(j)} + e_{t-1}^{(j)})\| \leq (1-\delta_g) (\|\Delta_{t-1}^{(j)}\| + \|e_{t-1}^{(j)}\|) \leq \sum_{k = 1}^{t-1} (1-\delta_g)^{t-k} \|\Delta_k^{(j)}\|.
\]

When $t_1<t_2$, it holds that:
\begin{align*}
    E(\Delta_{t_1}^{(i)}\Delta_{t_2}^{(j)}) &= E(E(\Delta_{t_1}^{(i)}\Delta_{t_2}^{(j)}|x_{t_2}))= E(E(\Delta_{t_1}^{(i)}|x_{t_2})E(\Delta_{t_2}^{(j)}|x_{t_2})) \\
&= E(E(\Delta_{t_1}^{(i)}|x_{t_2})E(\Delta_{t_2}^{(i)}|x_{t_2})) =E(E(\Delta_{t_1}^{(i)}\Delta_{t_2}^{(i)})|x_{t_2})\\
&=E(\Delta_{t_1}^{(i)}\Delta_{t_2}^{(i)}),
\end{align*}
where the equalities hold since worker i and worker j work in the same setting and independently.
%
%On the other hand, when $t_1=t_2, i\neq j$, since workers $i$ and $j$ work independently, it holds that
%\begin{align*}
%    E(\Delta_{t_1}^{(i)}\Delta_{t_2}^{(j)}) 
%&= E(\Delta_{t_1}^{(i)})E(\Delta_{t_2}^{(j)}) = E(\Delta_{t_1}^{(i)})^2 \leq E([\Delta_{t_1}^{(i)}]^2).
%\end{align*} 

Then, we have 
\[
\begin{split}
\mathbb{E}\left[\frac{1}{N^2}\sum_{t=1}^T\sum_{i=1}^N\sum_{j=1}^N \|e_t^{(i)}\|\|\Delta_t^{(j)}\|\right] &\leq
\mathbb{E}\left[\frac{1}{N^2}\sum_{t=1}^T\sum_{i=1}^N\sum_{j=1}^N\sum_{k=1}^{t-1} (1-\delta_g)^{t-k}\|\Delta_k^{(i)}\|\|\Delta_t^{(j)}\|\right]\\
&\leq \mathbb{E}\left[\frac{1}{N}\sum_{t=1}^T\sum_{k=1}^{t-1}\sum_{i=1}^N(1-\delta_g)^{t-k} \|\Delta_k^{(i)}\|\|\Delta_t^{(i)}\|\right]\\
&\leq \frac{1-\delta_g}{\delta_gN}\sum_{t=1}^T\sum_{i=1}^N \mathbb{E}\|\Delta_t^{(i)}\|^2,
\end{split}
\]
where the last inequality can be proven by Lemma \ref{matrix}. Hence, the proof is completed.
\end{proof}

\begin{lemma}
Let $e_t$ be the noisy term defined in Algorithm \ref{alg1} and $\Delta^{(i)}_t$ be the term defined in Notation \ref{notation-thm2}. Then it holds that 
\[
\mathbb{E}\left[\frac{1}{N}\sum_{t=1}^T\sum_{i=1}^N\|e_t\|\|\Delta_t^{(i)}\|\right] \leq \frac{(1-\delta_x)(2-\delta_g)}{N\delta_x\delta_g}\sum_{i=1}^N \mathbb{E}\left[\sum_{t=1}^T\|\Delta_t^{(i)}\|^2\right]
\]
\end{lemma}
\begin{proof}
With the definition of $e_t$, we obtain
\[
\begin{split}
\|e_t\| &= \|\hat{\delta}_{t-1} + e_{t-1} - Q_x(\hat{\delta}_{t-1} + e_{t-1})\| \leq (1-\delta_x)(\|\hat{\delta}_{t-1}\| + \|e_{t-1}\|)\\
 &=(1-\delta_x)\left(\frac{1}{N}\left\|\sum_{j = 1}^N Q_g(\Delta_{t-1}^{(j)} + e_{t-1}^{(j)})\right\| + \|e_{t-1}\|\right)\\ 
 &\leq (1-\delta_x)\left(\frac{1}{N}\left\|\sum_{j = 1}^N Q_g(\Delta_{t-1}^{(j)} + e_{t-1}^{(j)}) - \Delta_{t-1}^{(j)} + e_{t-1}^{(j)}\right\| +\frac{1}{N}\sum_{j=1}^N\|\Delta_{t-1}^{(j)} + e_{t-1}^{(j)}\| + \|e_{t-1}\|\right)\\
 &\leq (1-\delta_x)\left(\frac{2-\delta_g}{N}\sum_{j=1}^N\|\Delta_{t-1}^{(j)}\| + \frac{2-\delta_g}{N}\sum_{j=1}^N\|e_{t-1}^{(j)}\| + \|e_{t-1}\|\right) \\
&\leq \frac{1}{N}(1-\delta_x)((2-\delta_g)\sum_{j=1}^N\|\Delta_{t-1}^{(j)}\| + (2-\delta_g)\sum_{j=1}^N\sum_{k=1}^{t-1}(1-\delta_g)^{t-k}\|\Delta_k^{(j)}\| + \|e_{t-1}\|)\\
&\leq \frac{1}{N}\sum_{l=1}^{t-1} (1-\delta_x)^{t-l}(2-\delta_g)(\sum_{j=1}^N\|\Delta_l^{(j)}\| + \sum_{j=1}^N\sum_{k = 1}^{l-1} (1-\delta_g)^{l-k}\|\Delta_k^{(j)}\|)
\end{split} 
\]

Besides, for sequence $\{a_i\}$, we have
\[
\begin{split}
\sum_{t=1}^T\sum_{l=1}^{t-1}\sum_{k=1}^{l-1} (1-\delta_x)^{t-l}(1-\delta_g)^{l-k}a_ka_t &= \sum_{t=1}^T\sum_{k=1}^{t-1}\sum_{l=k+1}^{t-1} (1-\delta_x)^{t-l}(1-\delta_g)^{l-k}a_ka_t\\
\end{split}
\]

By similar construction of matrix in Lemma \ref{matrix}, we get the matrix U, where
$U_{i,j} = \frac{1}{2}\sum_{l=min(i,j)+1}^{max(i,j)-1}(1-\delta_x)^{max(i,j)-l}(1-\delta_g)^{l-min(i,j)}$ for $i\neq j$, and $U_{i,i} = 0$.

Therefore $U_{\infty}\leq 2*\frac{1}{2} \sum_{t=1}^T \sum_{l=t+1}^{T-1} (1-\delta_x)^{T-l} (1-\delta_g)^{l-t}\leq \frac{(1-\delta_x)(1-\delta_g)}{\delta_x\delta_g}$. 

So, we can get $\sum_{t=1}^T\sum_{l=1}^{t-1}\sum_{k=1}^{l-1} (1-\delta_x)^{t-l}(1-\delta_g)^{l-k}a_ka_t \leq  \frac{(1-\delta_x)(1-\delta_g)}{\delta_x\delta_g}\sum_{t=1}^T a_t^2$.

Because each worker works independently, by substituting the result in, we have
\[
\begin{split}
&\mathbb{E}\left[\frac{1}{N}\sum_{t=1}^T\sum_{i=1}^N\|e_t\|\|\Delta_t^{(i)}\|\right] \\
&\leq \mathbb{E}\left[\frac{1}{N^2}\sum_{t=1}^T\sum_{i=1}^N\sum_{l=1}^{t-1}\sum_{j=1}^N(1-\delta_x)^{t-l}(2-\delta_g)\left(\|\Delta_l^{(j)}\||\Delta_t^{(i)}\| + \sum_{k=1}^{l-1}(1-\delta_g)^{l-k}\|\Delta_k^{(j)}\|\|\Delta_t^{(i)}\|\right)\right]\\
&\leq \mathbb{E}\left[\frac{1}{N} \sum_{t=1}^T\sum_{i=1}^N\sum_{l=1}^{t-1} (1-\delta_x)^{t-l}(2-\delta_g)\left(\|\Delta_l^{(i)}\|\|\Delta_t^{(i)}\| + \sum_{k=1}^{l-1}(1-\delta_g)^{l-k}\|\Delta_k^{(i)}\|\|\Delta_t^{(i)}\|\right)\right]\\
&\leq \mathbb{E}\left[\frac{(1-\delta_x)(2-\delta_g)}{N\delta_x}\sum_{t=1}^T\sum_{i=1}^N\|\Delta_t^{(i)}\|^2 + \frac{(1-\delta_x)(1-\delta_g)(2-\delta_g)}{N\delta_x\delta_g}\sum_{t=1}^T\sum_{i=1}^N\|\Delta_t^{(i)}\|^2\right]\\
& = \mathbb{E}\left[\frac{(1-\delta_x)(2-\delta_g)}{N\delta_x\delta_g}\sum_{t=1}^T\sum_{i=1}^N\|\Delta_t^{(i)}\|^2\right]
\end{split}
\]
\end{proof}

\begin{lemma}\label{Mtmul}
By the definition of $M_t$, it holds that 
\[
\sum_{t=1}^T M_t \leq C_4d\alpha\left(\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right)- \frac{1-\beta}{2N}\sum_{i=1}^N\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t^{(i)}}^2,
\]
where 
\[
\begin{split}
C_2 &= \left(\frac{\beta/(1-\beta)}{\sqrt{C_1(1-\gamma)\theta_1}}+1\right)^2\\
C_4 &= \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})} \left(\frac{\alpha L(2-\delta_x)(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_x\delta_g} + \frac{2C_2G}{\sqrt{\theta}}\right)
\end{split}
\]
\end{lemma}
\begin{proof}
Similar to Lemma \ref{Mt}, we define $A_t^{(i)}$ and $B_t^{(i)}$ as follows:
\[
\begin{split}
A_t^{(i)} &= \frac{\beta m_{t-1}^{(i)}}{\sqrt{v_t^{(i)}}+\sqrt{\theta_tv_{t-1}^{(i)}}} - \frac{(1-\beta)g_t^{(i)}}{\sqrt{v_t^{(i)}}+\sqrt{\hat{v}_t^{(i)}}},\\
B_t^{(i)} &= \left(\frac{\beta m_{t-1}^{(i)}}{\sqrt{\theta_t v_{t-1}^{(i)}}} \frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}} +\sqrt{\theta_tv_{t-1}^{(i)}}}\frac{(1-\theta_t)\sigma_t^{(i)}}{\sqrt{\hat{v}_t^{(i)}} + \sqrt{\theta_tv_{t-1}^{(i)}}}\right) + \frac{(1-\beta)\sigma_t^{(i)}}{\sqrt{v_t^{(i)}}+\sqrt{\hat{v}_t^{(i)}}}.
\end{split}
\]

Still,  we can split $\mathbb{E}\langle \nabla f(x_t),\Delta_t\rangle$ into four terms:
\[
\begin{split}
\mathbb{E}\langle \nabla f(x_t),\Delta_t\rangle &= \frac{\beta\alpha_t}{\sqrt{\theta_t}\alpha_{t-1}}\mathbb{E}\langle \nabla f(x_t),\Delta_{t-1}\rangle - \frac{1}{N}\sum_{i=1}^N \mathbb{E}\langle \nabla f(x_t), (1-\beta)\hat{\eta}_t^{(i)} g_t^{(i)}\rangle \\
& \qquad - \frac{1}{N}\sum_{i=1}^N\mathbb{E}\left\langle \nabla f(x_t), \hat{\eta}_t^{(i)}g_t^{(i)}\frac{(1-\theta_t)g_t^{(i)}}{\sqrt{v_t^{(i)}}}A_t^{(i)} \right\rangle\\ &\qquad- \frac{1}{N} \sum_{i=1}^N \mathbb{E}\left \langle \nabla f(x_t), \hat{\eta}_t^{(i)}\sigma_t^{(i)}\frac{(1-\theta_t)g_i^{(i)}}{\sqrt{v_t^{(i)}}}B_t^{(i)}\right\rangle 
\end{split}
\]

For the first term, we obtain
\[
\begin{split}
\mathbb{E}\langle \nabla f(x_t),\Delta_{t-1}\rangle  &= \mathbb{E}\langle \nabla f(x_{t-1}),\Delta_{t-1}\rangle + \mathbb{E}\langle \nabla f(x_t)-\nabla f(x_{t-1}),\Delta_{t-1}\rangle\\
&\leq \mathbb{E}\langle \nabla f(x_{t-1}),\Delta_{t-1}\rangle + \mathbb{E} \|\nabla f(x_t)-\nabla f(x_{t-1})\|\|\Delta_{t-1}\|\\
&\leq \mathbb{E}\langle \nabla f(x_{t-1}),\Delta_{t-1}\rangle + L\mathbb{E} \left\|Q_x\left(\frac{1}{N}\sum_{i=1}^N Q_g(\Delta_{t-1}^{(i)}+e_{t-1}^{(i)}) +e_{t-1}\right)\right\|\|\Delta_{t-1}\|\\
&\leq \mathbb{E}\langle \nabla f(x_{t-1}),\Delta_{t-1}\rangle + L(2-\delta_x)\mathbb{E} \left\|\frac{1}{N}\sum_{i=1}^N Q_g(\Delta_{t-1}^{(i)}+e_{t-1}^{(i)}) +e_{t-1}\right\|\|\Delta_{t-1}\|\\
&\leq \mathbb{E}\langle \nabla f(x_{t-1}),\Delta_{t-1}\rangle + L(2-\delta_x)\mathbb{E}\|e_{t-1}\|\|\Delta_{t-1}\|\\&\qquad + L(2-\delta_x)(2-\delta_g) \frac{1}{N}\sum_{i=1}^N \|\Delta_{t-1}^{(i)}\|\|\Delta_{t-1}\|+ L(2-\delta_x)(2-\delta_g)\mathbb{E}\frac{1}{N}\sum_{i=1}^N\|e_{t-1}^{(i)}\|\|\Delta_{t-1}\|\\
&\leq \mathbb{E}\langle \nabla f(x_{t-1}),\Delta_{t-1}\rangle + \frac{L(2-\delta_x)}{N}\sum_{i=1}^N \mathbb{E}\|e_{t-1}\|\|\Delta_{t-1}^{(i)}\|
\\&\qquad +  \frac{L(2-\delta_x)(2-\delta_g)}{N}\sum_{i=1}^N \mathbb{E}\|\Delta_{t-1}^{(i)}\|^2+ \frac{L(2-\delta_x)(2-\delta_g)}{N^2}\mathbb{E}\sum_{i=1}^N\sum_{j=1}^N\|e_{t-1}^{(i)}\|\|\Delta_{t-1}^{(j)}\|\\
&=M_{t-1}.
\end{split}
\]

The second term remain the same as it is in the lemma \ref{Mt}, in which we obtain
\[
-\frac{1}{N}\sum_{i=1}^N\mathbb{E}\langle \nabla f(x_t),(1-\beta)\hat{\eta}_t^{(i)}g_t^{(i)}\rangle = -\frac{1-\beta}{N}\sum_{i=1}^N \|\nabla f(x_t)\|_{\hat{\eta}_t^{(i)}}^2.
\]

The third term can have similar derivation as it is in the lemma \ref{Mt}, we obtain
\[
-\frac{1}{N}\mathbb{E}\sum_{i=1}^N\left\langle \nabla f(x_t), \hat{\eta}_t^{(i)}g_t^{(i)}\frac{(1-\theta_t)g_t^{(i)}}{\sqrt{v_t^{(i)}}}A_t\right\rangle \leq \frac{1}{N}\sum_{i=1}^N \frac{1-\beta}{4}\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t^{(i)}}^2 + \frac{C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}}}\right\|^2.
\]

And for the fourth term, we have
\[
- \frac{1}{N} \sum_{i=1}^N \mathbb{E}\left \langle \nabla f(x_t), \hat{\eta}_t^{(i)}\sigma_t^{(i)}\frac{(1-\theta_t)g_i^{(i)}}{\sqrt{v_t^{(i)}}}B_t^{(i)}\right\rangle \leq \frac{1}{N}\sum_{i=1}^N \frac{1-\beta}{4}\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t^{(i)}}^2 + \frac{C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}}}\right\|^2.
\] 

By defining $N_t =  \frac{L(2-\delta_x)}{N}\sum_{i=1}^N \mathbb{E}\|e_{t}\|\|\Delta_{t}^{(i)}\|
+  \frac{L(2-\delta_x)(2-\delta_g)}{N}\sum_{i=1}^N \mathbb{E}\|\Delta_{t}^{(i)}\|^2+ \frac{L(2-\delta_x)(2-\delta_g)}{N^2}\mathbb{E}\sum_{i=1}^N\sum_{j=1}^N\|e_{t}^{(i)}\|\|\Delta_{t}^{(j)}\| + \frac{1}{N}\sum_{i=1}^N \frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}}}\right\|^2$, then with the same induction in Lemma \ref{Mt}, we obtain
\[
\begin{split}
\sum_{t=1}^T M_t \leq \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})}\sum_{t=1}^T N_t - \frac{1-\beta}{2N}\sum_{i=1}^N\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t^{(i)}}^2.
\end{split}
\]

Besides, we have
\[
\begin{split}
\sum_{t=1}^T N_t &= \sum_{t=1}^T \frac{L(2-\delta_x)}{N}\sum_{i=1}^N \mathbb{E}\|e_{t}\|\|\Delta_{t}^{(i)}\|
+  \frac{L(2-\delta_x)(2-\delta_g)}{N}\sum_{i=1}^N \mathbb{E}\|\Delta_{t}^{(i)}\|^2 \\&\qquad + \frac{L(2-\delta_x)(2-\delta_g)}{N^2}\mathbb{E}\sum_{i=1}^N\sum_{j=1}^N\|e_{t}^{(i)}\|\|\Delta_{t}^{(j)}\| + \frac{1}{N}\sum_{i=1}^N \frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}}}\right\|^2\\
&\leq \frac{L(2-\delta_x)(1-\delta_x)(2-\delta_g)}{N\delta_x\delta_g}\sum_{i=1}^N \sum_{t=1}^T \mathbb{E} \|\Delta_t^{(i)}\|^2 + \frac{L(2-\delta_x)(2-\delta_g)}{N}\sum_{t=1}^T\sum_{i=1}^N \mathbb{E}\|\Delta_{t}^{(i)}\|^2\\ &\qquad +\frac{L(2-\delta_x)(2-\delta_g)(1-\delta_g)}{\delta_gN}\sum_{i=1}^N \sum_{t=1}^T\mathbb{E}\|\Delta_t^{(i)}\|^2 +  \frac{1}{N}\sum_{i=1}^N \sum_{t=1}^T\frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}}}\right\|^2\\
& = \frac{L(2-\delta_x)(2-\delta_g)}{N\delta_x\delta_g}\sum_{i=1}^N \sum_{t=1}^T \mathbb{E} \|\Delta_t^{(i)}\|^2 +\frac{1}{N}\sum_{i=1}^N \sum_{t=1}^T\frac{2C_2G\alpha}{\sqrt{\theta}}\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}}}\right\|^2\\
&\leq \left(\frac{\alpha^2L(2-\delta_x)(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_x\delta_g} + \frac{2C_2G\alpha}{\sqrt{\theta}}\right) \frac{1}{N} \sum_{i=1}^N \sum_{t=1}^T\mathbb{E}\left\|\frac{\sqrt{1-\theta_t}g_t^{(i)}}{\sqrt{v_t^{(i)}}}\right\|^2\\
&\leq  \left(\frac{\alpha^2L(2-\delta_x)(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_x\delta_g} + \frac{2C_2G\alpha}{\sqrt{\theta}}\right) d\left[\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right]
\end{split}
\]

Combining the above two inequalities we can obtain the desired result.
\end{proof}

\begin{lemma}\label{multitau}
 Let $\tau$ be randomly chosen from $\{1,2,\cdots,T\}$ with equal probabilities $p_\tau = \frac{1}{T}$. We have the following estimate:
  \[
  \mathbb{E}[\|\nabla f(x_\tau)\|^2]\leq \frac{\sqrt{G^2+\epsilon d}}{\alpha\sqrt{T}N}\sum_{i=1}^N\mathbb{E}\left[\sum_{t=1}^T\|\nabla f((x_t))\|_{\hat{\eta_t}^{(i)}}^2\right].
  \]
\end{lemma}
\begin{proof}
  By Lemma \ref{ft}, $\mathbb{E}[\|\nabla f(x_\tau)\|^2]\leq \frac{\sqrt{G^2+\epsilon d}}{\alpha\sqrt{T}}\mathbb{E}[\sum_{t=1}^T\|\nabla f(x_t)\|_{\hat{\eta_t}^{(i)}}^2$ holds for any $i$. Hence, the proof is finished.
\end{proof}

\begin{proof}[Proof of Theorem \ref{T2}]
By using the gradient Lipschitz continuity of $f$, it holds that
\[
\begin{split}
\mathbb{E} f(\hat{x}_{t+1}) &\leq \mathbb{E}\left[f(\hat{x}_t) +\langle \nabla f(\hat{x}_t), \Delta_t\rangle + \frac{L}{2}\|\Delta_t\|^2 \right] \\
& = \mathbb{E}\left[f(\hat{x}_t) +\langle \nabla f(x_t), \Delta_t\rangle +\langle \nabla f(\hat{x}_t) - \nabla f(\tilde{x}_t), \Delta_t\rangle +\langle \nabla f(\tilde{x}_t) - \nabla f(x_t), \Delta_t\rangle + \frac{L}{2}\|\Delta_t\|^2 \right]\\
&\leq \mathbb{E}\left[f(\hat{x}_t) +\langle \nabla f(x_t), \Delta_t\rangle +L\|E_t\|\|\Delta_t\| +L\|e_t\|\|\Delta_t\| + \frac{L}{2}\|\Delta_t\|^2 \right]\\
&\leq \mathbb{E}\left[f(\hat{x}_t) +\langle \nabla f(x_t), \Delta_t\rangle +\frac{L(2-\delta_x)}{N}\sum_{i=1}^N \|e_{t}\|\|\Delta_{t}^{(i)}\| + \frac{L(2-\delta_x)(2-\delta_g)}{N}\sum_{i=1}^N \|\Delta_{t}^{(i)}\|^2 \right. \\  &\left.\qquad + \frac{L(2-\delta_x)(2-\delta_g)}{N^2}\sum_{i=1}^N\sum_{j=1}^N\|e_{t}^{(i)}\|\|\Delta_{t}^{(j)}\|\right]\\
&=\mathbb{E}f(\hat{x}_t) +M_t.
\end{split}
\]

Then by summing $t$ from $1$ to $T$, we obtain
\[
\begin{split}
f^*&\leq \mathbb{E}f(x_{T+1}) \leq f(x_1) + \sum_{t=1}^T M_t\\
&\leq f(x_1) +C_4d\alpha\left(\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right)- \frac{1-\beta}{2N}\sum_{i=1}^N\sum_{t=1}^T\mathbb{E}\|\nabla f(x_t)\|_{\hat{\eta}_t^{(i)}}^2,
\end{split}
\]

Using Lemma \ref{multitau} and arranging some terms, we have
\[
\begin{split}
\mathbb{E}[\|\nabla f(x_\tau)\|^2]&\leq \frac{\sqrt{G^2+\epsilon d}}{\alpha\sqrt{T}N}\sum_{i=1}^N\mathbb{E}\left[\sum_{t=1}^T\|\nabla f((x_t))\|_{\hat{\eta_t}^{(i)}}^2\right]\\
&\leq \frac{2\sqrt{G^2+\epsilon d}}{\alpha(1-\beta)\sqrt{T}} \left( f(x_1) - f^* +C_4d\alpha\left(\log\left(1+\frac{G^2}{\epsilon d}\right)+\frac{1}{1-\theta}\sum_{t=1}^T (1-\theta_t)\right)\right)\\
&\leq \frac{C_5+C_6\sum_{t=1}^T \frac{1}{t}}{\sqrt{T}},
\end{split}
\]

where 
\[
\begin{split}
C_2 &= \left(\frac{\beta/(1-\beta)}{\sqrt{C_1(1-\gamma)\theta_1}}+1\right)^2,\\
C_4 &= \frac{1}{\sqrt{C_1}(1-\sqrt{\gamma})} \left(\frac{\alpha L(2-\delta_x)(2-\delta_g)}{C_1\theta(1-\sqrt{\gamma})^2\delta_x\delta_g} + \frac{2C_2G}{\sqrt{\theta}}\right),\\
C_5 &= \frac{2\sqrt{G^2+\epsilon d}}{\alpha(1-\beta)}\left(f(x_1) - f^* + C_4d\alpha\log\left(1+\frac{G}{\epsilon d}\right)\right),\\
C_6 &= \frac{2\sqrt{G^2+\epsilon d}C_4 d}{(1-\beta)(1-\theta)}.\\
\end{split}
\]
\end{proof}

